Radio Foundation Models: Pre-training Transformers for 5G-based Indoor Localization

Artificial Intelligence (AI)-based radio fingerprinting (FP) outperforms classic localization methods in propagation environments with strong multipath effects. However, the model and data orchestration of FP are time-consuming and costly, as it requires many reference positions and extensive measurement campaigns for each environment. Instead, modern unsupervised and self-supervised learning schemes require less reference data for localization, but either their accuracy is low or they require additional sensor information, rendering them impractical. In this paper we propose a self-supervised learning framework that pre-trains a general transformer (TF) neural network on 5G channel measurements that we collect on-the-fly without expensive equipment. Our novel pretext task randomly masks and drops input information to learn to reconstruct it. So, it implicitly learns the spatiotemporal patterns and information of the propagation environment that enable FP-based localization. Most interestingly, when we optimize this pre-trained model for localization in a given environment, it achieves the accuracy of state-of-the-art methods but requires ten times less reference data and significantly reduces the time from training to operation.

==> src/graveyard.tex <==

% Knowing the wireless channel is becoming increasingly important for radio frequency (RF)-based applications, 
% including communication, localization and sensing~\cite{Bourdoux2020}. 
% While in the past the channel was considered as a source of interference, modern wideband systems allow us to 
% exploit channel characteristics, i.e., multipath components (MPCs), to improve the provided services. 

% Complex environments, such as industrial facilities, exhibit wireless channels with dense multipath and 
% non-line-of-sight (NLOS) conditions, 
% which reduces the performance of conventional channel parameter estimators such as MUSIC.
% % The assumptions that are made by classical channel parameter estimators often do not hold under harsh conditions such as
% % dense multipath.
% Hence, new approaches have to be developed that incorporate complex effects.
% Recent works~\cite{Kram2022, Ott2023} show that methods based on deep neural networks (DNN), trained in a
% supervised manner, outperform conventional channel parameter estimators. 


% We consider an environment with $N_{an}$ antennas (anchors) placed at known fixed positions 
% $\boldsymbol{p}_{an, i}$ with $i \in \{1\dots N_{an}\}$. 
% A target, equipped with an transmitter, moves around the environment and periodically sends a wideband ranging signal $s(t)$.
% In pretraining, we don't know the target position. 
% In finetuning, we assume we have measurements at known positions. 

% The simultaneously measured channel measurements $r(t)$ at the anchors are described by the 
% outcome of transmitting $s(t)$ over the channel $h(t)$ plus additive white noise $w(t)$: 
% \begin{equation}
%     r(t) = s(t) * h(t) + w(t),
% \end{equation}
% The channel is characterized by the amplitudes $\alpha_m$ and delays $T_m$ of the $m$ multipath components (MPCs) 
% which in turn are highly dependent on the properties of the environment, i.e., the geometry and surface materials.
% We describe the channel impulse response (CIR) such that 
% \begin{equation}
%         h(t) = \sum_{m} \alpha_{m}\delta(t-T_{m}),
% \label{eq:chmod1}   
% \end{equation}
% where $\delta$ is the dirac delta function.
% We generate an CIR estimate at each anchor by applying the autocorrelation: 
% \begin{equation}
% \hat h_i(\tau) = \int_{-\infty}^{\infty} r(t)s^*(t - \tau)\,dt.
% \end{equation}
% Finally, we combine the discrete-time CIR estimates $\boldsymbol{\hat h}_i$ into a matrix such that
% \begin{equation}
% \boldsymbol{\hat H} = \begin{bmatrix} \boldsymbol{\hat h}_0 \\ \vdots \\ \boldsymbol{\hat h}_{N_{an}-1}\end{bmatrix} 
% \end{equation}
% The idea is to exploit the pattern and correlations in the combined CIRs $\boldsymbol{\hat H}$, which are highly 
% characteristic for a certain position in the environment.



% Before we feed them into the transformer, each time step of the raw CIRs 
% (see Figure~\ref{fig:overview_method} grey blocks) are embedded in latent space via a learned linear projection.
% The embedding consists of $d_{model}$ dimensions.
% Figure~\ref{fig:overview_method} shows the input embedding as dark blue boxes. 
% Our strategy optimizes the embedding to maximize the amount of information the 
% attention mechanism can capture. 
% Attention determines how much each input position  
% contributes to the computation of the representation along a single dimension 
% (commonly along the time dimension for signals).
% Consequently, the ability to resolve long distance relationships in the data is limited 
% to this dimension.
% In our case the raw data is naturally three dimensional including the time and antenna dimensions 
% as well as a dimension that splits the complex signal into real and imaginary part.
% However, we want to find pattern in the signals across both, the antenna and time dimensions. 
% Hence, we vectorize them such that the CIRs are lined up along the attention dimension.
% This results in an input sequence of length $l_sN_{an}$ where $l_s$ is the length of each CIR.
% Figure~\ref{fig:embedding} shows how we combine the CIRs from three antennas.
% Due to this arrangement, it is possible to attend (indicated by dotted lines) to features 
% across all antennas. 
% \begin{figure}[tb!]
%     \centering
%     \includegraphics[width=3.5in]{figures/embedding.png}
%     \caption{Caption}
%     \label{fig:embedding}
% \end{figure}
